CyberMentor: AI Powered Learning Tool Platform to Address Diverse Student Needs in Cybersecurity Education

Many non-traditional students in cybersecurity programs often lack access to advice from peers, family members and professors, which can hinder their educational experiences. Additionally, these students may not fully benefit from various LLM-powered AI assistants due to issues like content relevance, locality of advice, minimum expertise, and timing. This paper addresses these challenges by introducing an application designed to provide comprehensive support by answering questions related to knowledge, skills, and career preparation advice tailored to the needs of these students. We developed a learning tool platform, CyberMentor, to address the diverse needs and pain points of students majoring in cybersecurity. Powered by agentic workflow and Generative Large Language Models (LLMs), the platform leverages Retrieval-Augmented Generation (RAG) for accurate and contextually relevant information retrieval to achieve accessibility and personalization. We demonstrated its value in addressing knowledge requirements for cybersecurity education and for career marketability, in tackling skill requirements for analytical and programming assignments, and in delivering real time on demand learning support. Using three use scenarios, we showcased CyberMentor in facilitating knowledge acquisition and career preparation and providing seamless skill-based guidance and support. We also employed the LangChain prompt-based evaluation methodology to evaluate the platform's impact, confirming its strong performance in helpfulness, correctness, and completeness. These results underscore the system's ability to support students in developing practical cybersecurity skills while improving equity and sustainability within higher education. Furthermore, CyberMentor's open-source design allows for adaptation across other disciplines, fostering educational innovation and broadening its potential impact.

==> appendex/appendex_hyperparameter.tex <==
\section{Hyper-parameters in LLMs}

In this research paper, we choose and compare three popular LLMs models: \texttt{gpt-3.5-turbo-1106}, \texttt{gpt-4-1106-preview}, \texttt{gemini-pro}. The details configurations can be found at Table \ref{tab:hyper_parameters}. We set the maximum token limit to 4096, allowing for extensive and detailed responses. Our experiments were conducted with a single response output (\(n=1\)), ensuring focused and specific replies and each LeetCode question will only generate one code solution. To balance creativity with relevance, we adjusted the temperature to 0.5, a moderate setting that encourages a mix of predictable and innovative responses. The \texttt{top\_p} parameter was set to 1, enabling the model to consider the full range of possible next words. We applied a frequency penalty of 0.0 to prevent repetition and a presence penalty of 0.6, encouraging the model to introduce new concepts and ideas throughout the conversation. This configuration was pivotal in achieving the desired balance between coherence, relevance, and novelty in the model's responses. 


\begin{table}
\centering
\caption{Hyper-Parameter of LLMs}

\begin{tabular}
    {
    >{\centering\arraybackslash}m{3cm}
      >{\centering\arraybackslash}m{4cm}
    }  

\hline
\textbf{Parameter} & \textbf{Models}\\ 
\hline
    Engine                & gpt-4-1106-preview,  gpt-3.5-turbo-1106, gemini-pro\\ \hline
  Max Token & 4096 \\ \hline
  n (responses) & 1 \\ \hline
  Temperature & 0.5 \\ \hline
  Top P & 1 \\ \hline
  Frequency Penalty & 0 \\ \hline
  Presentation Penalty & 0.6 \\ \hline\end{tabular}
\label{tab:hyper_parameters}
\end{table}


\begin{comment}
\begin{table*}
\centering
\caption{Hyper-parameter of LLMs}
\begin{tabular}{|r|l|l|l|}
\hline
\textbf{Parameter}    & \multicolumn{3}{|c|}{\textbf{Models}}\\ \hline
    Engine                & gpt-4-1106-preview& gpt-3.5-turbo-1106&gemini-pro\\ \hline
    Max Tokens            & \multicolumn{3}{|c|}{4096}\\ \hline
    n                     & \multicolumn{3}{|c|}{1}\\ \hline
    Temperature           & \multicolumn{3}{|c|}{0.5}\\ \hline
    Top P                 & \multicolumn{3}{|c|}{1}\\ \hline
    Frequency Penalty     & \multicolumn{3}{|c|}{0}\\ \hline
    Presence Penalty      & \multicolumn{3}{|c|}{0.6}\\ \hline
\end{tabular}
\label{tab:hyper_parameters}
\end{table*}
\end{comment}

==> appendex/guideline_general.tex <==
\section{General Guidelines for High-Quality Python Code}

\begin{itemize}
    \item \textbf{Understand the Problem and Edge Cases}: Before coding, make sure you fully understand the problem, including its edge cases. This understanding guides your approach and helps prevent oversights.
    \item \textbf{Choose the Right Data Structures}: Efficient data structures are key in solving LeetCode problems. Understand when to use arrays, sets, dictionaries, heaps, or other data structures based on the problem's requirements.
    \item \textbf{Optimize Algorithms for Performance}: Focus on algorithms that minimize time and space complexity. LeetCode problems often test your ability to find efficient solutions.
    \item \textbf{Write Clean and Concise Code}: LeetCode solutions should be straightforward and concise. Avoid unnecessary complexity in both logic and code structure.
    \item \textbf{Use Python Built-in Functions and Libraries}: Python's standard library offers many built-in functions that can simplify your code and make it more efficient, like sorted(), max(), min(), and list comprehensions.
    \item \textbf{Error Handling and Input Validation}: While LeetCode typically provides valid inputs, understanding how to handle errors and validate inputs is a good practice, especially for real-world applications.
    \item \textbf{Modularize Code with Functions}: Break your solution into functions or methods, each handling a specific part of the task. This makes your code more readable and easier to debug.
    \item \textbf{Document Your Approach with Comment}s: Use comments to explain your approach, especially if the algorithm is complex. This practice is useful for your future reference and for others who might read your code.
    \item \textbf{Test Your Code with Different Cases}: Before submitting, test your solution with various test cases, including edge cases, to ensure its correctness and efficiency.
    \item \textbf{Analyze Time and Space Complexity}: Always analyze the time and space complexity of your solution. Understanding Big O notation is crucial for optimizing LeetCode solutions and discussing them during interviews.
\end{itemize}


==> appendex/guideline_special.tex <==
\section{Specific Guidelines for High-Quality Python Code}

\begin{itemize}
    \item \textbf{Class Encapsulation:} Use classes and objects to encapsulate data and methods, promoting modularity and object-oriented design. \\
    \textit{Example:} For LeetCode question, code solution starts with \texttt{class Solution(): def ...}

    \item \textbf{Use of Standard Libraries:} The code effectively utilizes Python's standard libraries such as \texttt{re} (for regular expressions), \texttt{heapq} (for heap queue algorithms), \texttt{bisect} (for array bisection algorithms), and \texttt{math}. \\
    \textit{Best Practice:} Always prefer standard libraries over custom implementations for common algorithms, as they are optimized and well-tested.

    \item \textbf{Data Structures:} In Python and other programming languages, Node, ListNode, TreeNode are fundamental building blocks for linked lists and binary trees, essential for representing hierarchical or sequential data. Stack implements a basic stack data structure, useful for scenarios requiring last-in-first-out (LIFO) operations like parsing expressions or depth-first search. \\
    \textit{Best Practice:} Choose the right data structure based on the problem requirements for efficiency in both time and space complexity.

    \item \textbf{Itertools Usage:} Itertools is a powerful module in Python that offers a suite of functions designed to work on iterators. Using itertools in coding for permutations, combinations, and cartesian products is a sign of advanced Python knowledge, crucial for solving combinatorial problems. \\
    \textit{Best Practice:} Leverage itertools to write cleaner and more efficient looping constructs.

    \item \textbf{Heap Queue (heapq):} The heapq module is used for implementing priority queues, vital in algorithms where you need to repeatedly access the smallest or largest element. \\
    \textit{Best Practice:} Use heapq for priority queue implementation instead of a sorted list for better performance.

    \item \textbf{Functional Programming:} Usage of functools like reduce, cache, and lru\_cache indicates a functional approach to problem-solving, efficient for operations that benefit from memoization or reducing a list. \\
    \textit{Best Practice:} Employ functional programming concepts where applicable to make the code more concise and readable.

    \item \textbf{Math and Random Modules:} The inclusion of math for mathematical operations and random for random number generation is suitable for problems involving mathematical computations and stochastic processes. \\
    \textit{Best Practice:} Understand and utilize the vast array of functions provided by these modules to simplify complex calculations.

    \item \textbf{Efficiency and Optimization:} The use of bisect for binary searches and heapq for efficient element access in priority queues shows an understanding of algorithmic efficiency. \\
    \textit{Best Practice:} Always consider time and space complexity; optimize code where necessary but avoid premature optimization.

    \item \textbf{Testing and Validation:} Make sure to pass the testing cases in if has any to ensure they work as expected under various scenarios. \\
    \textit{Best Practice:} Pass testing input and expected output.
\end{itemize}


==> appendex/prompts.tex <==
\section{Prompts}
\label{section:prompt}
Within the domain of LLMs, such as the entity engaged in the current interaction, the terminologies "system prompts" and "user prompts" delineate distinct categories of input stimuli instrumental in directing the model's output generation.

\begin{itemize}
    \item \textbf{System Prompt}: The system prompt is used to define the persona that LLM will play.  In our application, it is part of the system's design to help guide the LLM in generating responses or performing code generation to ensure it plays as a sophisticated programmer professional or mentor. 
    \item \textbf{User prompts}: They are the prompts specifying the questions, commands, or statements that users input into the system to seek a response from the LLM (played as a programming tutor). In essence, this encompasses the textual or verbal input furnished by the user to the model.
\end{itemize}

The following presents two illustrative examples of prompts utilized within the scope of our manuscript.

\begin{mybox}{An Example of System Prompt: Guru for Python Programming}
You are a professional Python tutor and assistant, skilled in crafting original, high-quality code. Your responses will be composed entirely of original code, avoiding the use of copied or pre-existing online sources, and will be presented without comments or explanatory text. When provided with our chat history and any specific directions from me: 
\begin{enumerate}
    \item Your primary goal is to assist students in refining and improving the code already discussed in our chat history, rather than devising entirely new code.
    \item You will adeptly modify and enhance the existing code in accordance with my guidelines.
\end{enumerate}
\end{mybox}


\begin{userpromptbox}{An Example of User Prompt: Guru for Python Programming}
Write Python 3 function \{\texttt{function\_name}\}() to solve: 
\begin{enumerate}
    \item \{\textbf{question}\}
    \item \{\textbf{chat\_history}\} + and also meets the testing cases: + \{\textbf{test\_cases}\}
    \item \{\textbf{chat\_history}\} + and also follows the code guidelines: + \{\textbf{guide\_general}\}
    \item \{\textbf{chat\_history}\} + and also follows the specific code guidelines: + \{\textbf{guide\_specific}\}
\end{enumerate}
\end{userpromptbox}



==> knowledge_documents/links.tex <==
https://www.knowledgehut.com/blog/security/ceh-vs-cissp



==> reference/links.tex <==
Planner:

https://github.com/langchain-ai/langgraph/blob/main/examples/plan-and-execute/plan-and-execute.ipynb?ref=blog.langchain.dev



==> sections/abstract.tex <==
\begin{abstract}

% need to update after the body of paper
This study explores the capacity of Large Language Models (LLMs) to potentially produce high-quality language code, more specifically Python, for educational applications. We utilize a step-by-step prompt refinement process through multiple rounds of dialogue interaction with three leading LLM models: Gemini Pro, ChatGPT 3.5, and ChatGPT 4. We mimic the incremental learning process of real-world language learning and code quality improvement procedures. Our analysis demonstrates that iterative problem-solving and code refinement using prompt engineering remarkably improve code quality. The enhancements are quantitatively confirmed by an existing code evaluator, indicating that well-crafted and structured prompts yield better code outputs. Without proper LLM prompt design, our study revealed the low quality of the LLM code generated using the LeetCode dataset\footnote{https://leetcode.com/}. We delved into more advanced prompting methods for enhancing code quality through different prompt engineering strategies. Notably, the premier model among the LLMs under scrutiny exhibited a pass rate (defined as the code functioning correctly) enhancement from 27\% to 71\%. We suggest that with problem-focused prompting practice, LLMs could significantly impact computer science education, developing more sophisticated and effective educational tools for both students and instructors.
\end{abstract}


==> sections/conclusion.tex <==
\section{Conclusion}
\label{section:conclusion}
In this study, we developed a novel learning system utilizing LLMs to generate Python code using the coding tasks from LeetCode. By employing a series of iterative prompt engineering strategies, we systematically improved the quality of the generated code for all three leading LLMs: Gemini Pro, ChatGPT 3.5, and ChatGPT 4. A key finding from our research is the significant improvement in code quality through multi-round dialog prompt engineering. Specifically, the most advanced model among those evaluated, ChatGPT 4, demonstrated a substantial increase in pass rates—from 27\% to 54\% using a single-round model, and further to 71\% with a multi-round dialog model. This enhancement not only underscores the effectiveness of refined prompt engineering but also highlights the potential of LLMs in educational applications. In addition, our experiments revealed that ChatGPT 4 excelled in both accuracy and time efficiency. This performance showcases the model's capability to support educational endeavors, particularly in the realm of computer programming.

Looking ahead, our research lays the groundwork for innovative learning methodologies within computer programming classes. We intend to extend our foundational model to create a comprehensive LLM-based chatbot. This chatbot will serve as a versatile Computer Science assistant, offering extensive support to both students and instructors. Its functionalities will not be limited to improving coding proficiency but will also include facilitating the teaching of computer programming courses, thus marking a significant step forward in the integration of artificial intelligence into education.


==> sections/discussion.tex <==
\section{Discussion}
\label{section:discussion}


\subsection{Response Evaluators}

\subsection{Code Evaluators}
In the course of our investigation, we deployed two distinct code evaluation mechanisms: a widely recognized conventional evaluator alongside a meticulously fine-tuned deep learning model. The landscape of code assessment transcends mere metrics such as pass rates and CPU runtime. It is imperative to incorporate additional dimensions of evaluation that address the qualitative aspects of code, for example, maintainability, security posture, and susceptibility to code smells. These criteria gain paramount importance when contemplating the application of LLMs or AI for code generation within real-world production environments. 







==> sections/introduction.tex <==
\section{Introduction}\label{section:introduction}


% \begin{figure}[ht]
% \centering
% \includegraphics[width=8cm]{images/flowchart_challenges.png}
% \caption{Flowchart illustrating the common challenges for students}
% \label{fig:flowchart_challenge}
% \end{figure}

% \begin{figure}[ht]
% \begin{mybox}{Code Question}
% Given an array of integers \texttt{\textbf{nums}} and an integer target, return indices of the two numbers such that they add up to target. You may assume that each input would have exactly one solution, and you may not use the same element twice. You can return the answer in any order.

% \end{mybox}
% \caption{An Example of Coding Question}
% \label{fig:code_question}
% \end{figure}


In the rapidly evolving field of education, integrating advanced technologies such as Large Language Models (LLMs) has become pivotal in enhancing learning experiences and solving complex problems. The advent of LLMs has introduced novel approaches in various domains, particularly in programming education, where traditional teaching methods often fall short in addressing the dynamic and intricate nature of coding. This paper explores the implementation of an LLM Agentic Workflow to facilitate and improve programming education, aiming to bridge the gap between theoretical understanding and practical application.

The proposed workflow leverages LLMs to assist students in comprehending programming concepts, formulating solutions, and addressing code vulnerabilities through a structured process. The workflow is designed to guide learners from problem understanding to solution formulation, ensuring a comprehensive grasp of programming principles. The core components of this workflow are categorized into two main sections: Programming Guidelines and Code Generation and Validation.

\subsection*{Programming Guidelines}

\begin{enumerate}
    \item \textbf{Problem Understanding in Programming}: This initial phase focuses on helping students comprehend the given problem, emphasizing the importance of a clear problem statement and the underlying concepts.
    \item \textbf{Solution Formulation}: After understanding the problem, the workflow guides learners in devising appropriate solutions, leveraging LLMs to provide relevant suggestions and methodologies.
    \item \textbf{Problem Categorization and Key Considerations}: Here, the workflow categorizes the problem based on its nature (e.g., functional, non-functional) and highlights key considerations that must be addressed to ensure an effective solution.
    \item \textbf{Pre-Code Generation Cautions}: This part emphasizes the precautions and best practices to consider before generating code. It aims to prepare students to write secure and efficient code by addressing potential pitfalls and ensuring adherence to coding standards.
\end{enumerate}

\subsection*{Code Generation and Validation}

\begin{enumerate}
    \item \textbf{Code Generation and Review}: Utilizing LLMs, the workflow aids in the actual generation of code, followed by a thorough review process to refine and optimize the solution.
    \item \textbf{Post-Code Generation Vulnerability Assessment}: After code generation, this phase involves evaluating the generated code for potential vulnerabilities. It ensures the robustness and security of the solution by identifying and mitigating any risks.
    \item \textbf{Generation of Unit Tests and Comprehensive Testing}: To ensure the reliability and correctness of the code, this component focuses on generating unit tests and conducting comprehensive testing for the problem. This phase leverages LLMs to create effective test cases and ensures thorough validation of the solution.
\end{enumerate}




\begin{table*}[ht]
\centering
\caption{A Summary of Challenges in Traditional Programming Class}
\begin{tabular}{|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Role}}  & \multicolumn{1}{c|}{\textbf{Questions}}                                     & \multicolumn{1}{c|}{\textbf{Category}}   \\ \hline
\multirow{14}{*}{Students}           & How can students overcome shyness when asking questions in class?           & \multirow{2}{*}{In-Class Concerns}       \\ \cline{2-2}
                                     & How can they assess the relevance and quality of their questions?           &                                          \\ \cline{2-3} 
                                     & How can I understand new programming terms I come across?                   & \multirow{3}{*}{Question Understanding}  \\ \cline{2-2}
                                     & How do I figure out what a coding problem is asking for?                    &                                          \\ \cline{2-2}
                                     & How can I identify the type of coding problem I’m working on?               &                                          \\ \cline{2-3} 
                                     & What steps can I take to solve coding problems logically?                   & \multirow{2}{*}{Problem Solving}         \\ \cline{2-2}
                                     & How do I choose the right data structure for my code?                       &                                          \\ \cline{2-3} 
                                     & What are the key tips for writing code without syntax errors?               & \multirow{3}{*}{Syntax}                  \\ \cline{2-2}
                                     & Which syntax mistakes are common and how can I avoid them?                  &                                          \\ \cline{2-2}
                                     & How can I check my code for errors before I run it?                         &                                          \\ \cline{2-3} 
                                     & How can I make sure my code does what it’s supposed to do?                  & \multirow{2}{*}{Logic}                   \\ \cline{2-2}
                                     & What should I do to ensure my code passes all the tests?                    &                                          \\ \cline{2-3} 
                                     & What can I do to make my code concisely?                                    & \multirow{2}{*}{Optimization}            \\ \cline{2-2}
                                     & How can I improve my code to use less memory and run quicker?               &                                          \\ \hline
\multirow{10}{*}{Instructors}        & What can I do to make the most of the time I have to teach?                 & \multirow{2}{*}{Time Constraints}        \\ \cline{2-2}
                                     & How can I balance my time in teaching and researching?                      &                                          \\ \cline{2-3} 
                                     & What strategies can I use to keep students engaged?                         & \multirow{2}{*}{Engagement}              \\ \cline{2-2}
                                     & How can I make complex topics easier for students to understand?            &                                          \\ \cline{2-3} 
                                     & How can I meet the learning needs of both beginners and advanced students?  & \multirow{2}{*}{Varied Skill Levels}     \\ \cline{2-2}
                                     & What can I do to make the course useful for students at all levels?         &                                          \\ \cline{2-3} 
                                     & How can I give students feedback quickly and effectively?                   & \multirow{2}{*}{Assessment and Feedback} \\ \cline{2-2}
                                     & What’s an efficient way to grade assignments and provide useful comments?   &                                          \\ \cline{2-3} 
                                     & How can I keep my course up-to-date and relevant?                           & \multirow{2}{*}{Curriculum Update}       \\ \cline{2-2}
                                     & What are good ways to integrate new tools and methods into my teaching?     &                                          \\ \hline
\multirow{4}{*}{Teaching Assistants} & How can I help students find the answer without just telling them directly? & \multirow{2}{*}{Assistance}              \\ \cline{2-2}
                                     & How can I balance helping students with my own studies and research?        &                                          \\ \cline{2-3} 
                                     & How can I make sure I’m giving good help to students?                       & \multirow{2}{*}{Quality}                 \\ \cline{2-2}
                                     & What can I do to ensure all teaching assistants are consistently helpful?   &                                          \\ \hline
\end{tabular}
\label{table:challenges_in_class}
\end{table*}

% \begin{figure*}[ht]
% \centering
% \includegraphics[width=16cm]{images/flowchart_idea.png}
% \caption{Flowchart illustrating coding and learning process using LLMs}
% \label{fig:flowchart_idea}
% \end{figure*}

\begin{figure*}[ht]
\centering
\includegraphics[width=1\linewidth]{images/model.png}
\caption{Flowchart illustrating coding and learning process using LLMs}
\label{fig:model}
\end{figure*}


% buff
In the rapidly evolving field of Artificial Intelligence (AI), Large Language Models (LLMs) \cite{bommasani2021opportunities, touvron2023llama}, a breakthrough in AI, have shown remarkable potential in a variety of applications, including natural language processing, content creation, and more recently, in code generation. Numerous LLM models, such as ChatGPT and LLaM, have shown their capability to cater to a variety of task domains, ranging from question answering to the generation of code snippets \cite{radford2019language, bommasani2021opportunities, ouyang2022training, liu2023pre, touvron2023llama}. Furthermore, in the evolving landscape of computer science education, integrating advanced technologies has become increasingly pivotal. Many Integrated Development Environments (IDEs) have equipped with LLMs to generate code in software development tools, such as VS Code\footnote{https://code.visualstudio.com/}. As the demand for proficient programmers grows, so does the necessity for innovative and effective teaching methods. These usages of tools draw attention to developing software vulnerabilities and security concerns. \cite{asare2023github, pearce2022asleep, dakhel2023github}.

% % Challenges in problem solving
% In conventional computer programming education, pedagogical exchanges between instructors and students were primarily characterized by face-to-face lectures, written materials, and static digital content. Students are facing many challenges in their programming study, as illustrated in Fig. \ref{fig:flowchart_challenge}. During the engagement with coding questions, students frequently encountered obstacles, leading to a lack of understanding of the problem statement, an inability to decompose the problem into manageable sub-tasks, uncertainty regarding the appropriate data structures and coding syntax, and challenges in debugging, which in turn diminished their enthusiasm and perseverance in problem-solving. Furthermore, the aspect of code efficiency emerged as a critical consideration in their academic journey and subsequent professional engagements, such as coding interviews.

% % Challenges in interactions
% Although students had the opportunity to pose questions during class sessions, the time window for inquiries was rigidly restricted to the scheduled classroom hours. Compounding this issue, some students, due to shyness or lack of confidence, hesitated to ask questions in front of their peers, further impeding their learning experience. Instructors were compelled to modulate the teaching pace to accommodate the majority, adhering to the syllabus to ensure comprehensive coverage of requisite topics and knowledge, often at the cost of limiting out-of-class interactions. Although students had the opportunity to consult instructors during office hours or via electronic communication, such as emails or Learning Management Systems like Blackboard, responses were frequently delayed. This hindered students' capacity to promptly learn from their errors and impeded the pace of their academic advancement. Instructors, on the other hand, also faced challenges that the arduous tasks of manual grading and responding to individual student inquiries, which could encroach upon their ability to engage deeply in personalized instruction and the development of curricula that reflect the latest advancements in computer science education. While this traditional method had some efficacy, it lacked the required flexibility and immediacy of response.

% re-write pain points from three roles perspectives
In the realm of university-level computer programming education, traditional pedagogical approaches have manifested numerous challenges, impacting students, instructors, and teaching assistants alike. These challenges, summarized in Table \ref{table:challenges_in_class}, often accentuated in foundational courses like Python programming, underscore the necessity for an evolved teaching paradigm.

\begin{itemize}
    \item \textbf{Students}: frequently encounter barriers related to classroom dynamics and cognitive load. The reluctance to pose questions due to social apprehension or the fear of irrelevance often leads to a lack of clarity in understanding programming concepts and problem statements. Furthermore, the acquisition of new programming terminologies and the identification of problem types present considerable cognitive challenges. These issues, compounded with the intricacies of problem-solving, debugging, and code optimization, necessitate a structured and supportive learning environment. Students must navigate through these educational hurdles to develop proficiency in logical reasoning, syntax accuracy, and algorithmic efficiency, which are pivotal in crafting optimized and error-free code.
    \item \textbf{Instructors}: grapple with the dual challenges of time management and pedagogical effectiveness. The finite nature of class periods imposes constraints on the depth and breadth of content delivery, necessitating strategic planning to maximize instructional efficacy. Engaging diverse learner groups, each with varying levels of prior knowledge and learning speeds, further complicates the teaching process. Instructors must tailor their methodologies to foster an inclusive and comprehensible learning atmosphere. Moreover, the rapid evolution of programming technologies demands continual curriculum updates, posing an ongoing challenge in integrating contemporary tools and practices. This dynamic landscape requires instructors to maintain a delicate balance between instructional thoroughness and the adaptability of course content to current industry standards.
    \item \textbf{Teaching assistants (TAs)}: are pivotal in bridging the gap between student needs and instructional goals. Their role involves not only facilitating understanding but also fostering autonomy in learning, especially under constrained time conditions. The effectiveness of TAs is contingent upon their ability to provide consistent, high-quality assistance, necessitating a well-structured support framework. Concurrently, TAs must adeptly manage their academic and research commitments, highlighting the importance of proficient time management skills. This delicate juggling act underscores the necessity for TAs to cultivate organizational competencies and prioritization techniques, ensuring their dual roles of educator and scholar are both effectively executed.
\end{itemize}

% Our idea that helps to address the challenges using LLMs
Large Language Models (LLMs) like ChatGPT represent a promising frontier in addressing the perennial challenges of university-level programming education. Our research posits that LLMs can revolutionize the teaching and learning of fundamental programming languages, such as Python, by providing an interactive, adaptive, and personalized learning experience. The potential of LLMs to serve as both a knowledgeable assistant and an insightful tutor could redefine traditional education paradigms. In our approach, we will explore how LLMs can deliver tailored guidance and instant feedback on coding tasks, facilitating a deeper understanding of programming concepts through interactive examples and real-time debugging assistance. Our study aims to investigate the efficacy of LLMs in enhancing the problem-solving skills of students, reducing the instructional workload on educators, and providing scalable, individualized support. By integrating LLMs into the programming curriculum, we envision creating a more engaging and efficient learning environment that not only addresses the existing educational challenges but also inspires a new generation of programmers.

%\subsection{Paper Organization}, if pages limit, remove this paragraph
The remainder of this paper is structured as follows: Section~\ref{section:related_work} reviews related work, emphasizing prior research in this domain and our unique contributions. The research problem is explicitly framed in Section~\ref{section:problem_statement}. Section~\ref{section:methodology} elaborates on our methodologies and the design of our model. The findings from our experiments are analyzed in Section~\ref{section:result_analysis}. Discussions on the implications of these findings are presented in Section~\ref{section:discussion}. Finally, Section~\ref{section:conclusion} concludes the paper, summarizing our contributions.


==> sections/methodology.tex <==
\section{Methodology}
\label{section:methodology}


The implementation of the Agentic Workflow draws inspiration from the HuggingGPT framework, which effectively leverages LLMs to orchestrate and manage complex tasks. The Agentic Workflow is structured to provide continuous support and feedback to learners throughout the programming process. The key aspects of this implementation are:

\begin{enumerate}
    \item \textbf{Agent Orchestration}: The intelligent agent orchestrates the various stages of the workflow, ensuring a seamless transition from one phase to another. This orchestration is crucial for maintaining coherence and providing timely assistance.
    \item \textbf{Multi-Tasking Capabilities}: Similar to HuggingGPT, the agent is equipped with multi-tasking capabilities, enabling it to handle multiple queries and tasks simultaneously. This feature is particularly beneficial in a learning environment where students may have diverse and concurrent needs.
    \item \textbf{Dynamic Interaction}: The agent facilitates dynamic interaction with learners, allowing for real-time feedback and guidance. This interactive approach helps students to clarify doubts and receive immediate support, thereby enhancing their learning experience.
    \item \textbf{Resource Utilization}: The workflow utilizes various resources such as pre-trained models and domain-specific datasets to provide accurate and contextually relevant assistance. By leveraging these resources, the agent can offer high-quality support tailored to the specific needs of programming education.
    \item \textbf{Continuous Improvement}: Inspired by the iterative nature of HuggingGPT, the Agentic Workflow incorporates mechanisms for continuous improvement. Feedback from users is systematically collected and analyzed to refine the workflow and enhance its effectiveness over time.
\end{enumerate}

\subsection*{Examples of Workflow Application}

The effectiveness of the Agentic Workflow can be demonstrated through various examples. Below, we present two examples that illustrate the workflow’s application in different problem-solving scenarios.

\begin{table*}[ht]
\centering
\begin{tabular}{|p{0.45\textwidth}|p{0.45\textwidth}|}
\hline
\textbf{Reversing Nodes in a Linked List in Groups of k} & \textbf{Maximizing Social Distancing in Cows} \\
\hline
\textbf{Problem Breakdown:} & \textbf{Problem Breakdown:} \\
\begin{enumerate}
    \item \textbf{Understanding}:
    \begin{itemize}
        \item A linked list needs to be reversed in groups of \( k \).
        \item If the number of nodes is not a multiple of \( k \), the remaining nodes should remain as they are.
    \end{itemize}
    \item \textbf{Solution Formulation}:
    \begin{itemize}
        \item Traverse the list to count nodes and identify groups of \( k \).
        \item Reverse the nodes within each group.
        \item Ensure proper linking of the reversed groups with the remaining nodes.
    \end{itemize}
    \item \textbf{Pre-Code Generation Cautions}:
    \begin{itemize}
        \item Handle edge cases like small lists or lists where the number of nodes is not a multiple of \( k \).
        \item Ensure pointers are correctly updated to maintain list integrity.
    \end{itemize}
    \item \textbf{Code Generation and Review}:
    \begin{itemize}
        \item Generate the code to reverse nodes in groups.
        \item Review and optimize the generated code.
    \end{itemize}
    \item \textbf{Post-Code Generation Vulnerability Assessment}:
    \begin{itemize}
        \item Assess the code for potential vulnerabilities such as pointer mismanagement.
        \item Ensure that no nodes are lost or incorrectly linked.
    \end{itemize}
    \item \textbf{Unit Tests and Comprehensive Testing}:
    \begin{itemize}
        \item Generate unit tests to cover various edge cases and scenarios.
        \item Conduct comprehensive testing to validate the solution’s correctness and efficiency.
    \end{itemize}
\end{enumerate} & 
\begin{enumerate}
    \item \textbf{Understanding}:
    \begin{itemize}
        \item Farmer John wants to maximize \( D \), the distance between the closest two occupied stalls, after placing two new cows.
        \item The barn has \( N \) stalls, some of which are occupied.
    \end{itemize}
    \item \textbf{Solution Formulation}:
    \begin{itemize}
        \item Identify the currently occupied stalls.
        \item Determine the optimal placement of the two new cows to maximize \( D \).
        \item Ensure that no existing cows are moved.
    \end{itemize}
    \item \textbf{Pre-Code Generation Cautions}:
    \begin{itemize}
        \item Consider edge cases like all stalls being either occupied or vacant.
        \item Ensure that the placements are within the barn's boundaries.
    \end{itemize}
    \item \textbf{Code Generation and Review}:
    \begin{itemize}
        \item Generate the code to calculate \( D \) and determine optimal placements.
        \item Review and optimize the generated code for efficiency and correctness.
    \end{itemize}
    \item \textbf{Post-Code Generation Vulnerability Assessment}:
    \begin{itemize}
        \item Assess the code for potential vulnerabilities such as incorrect distance calculations.
        \item Ensure that the placement logic is sound and doesn't lead to invalid positions.
    \end{itemize}
    \item \textbf{Unit Tests and Comprehensive Testing}:
    \begin{itemize}
        \item Generate unit tests to cover various barn configurations and placements.
        \item Conduct comprehensive testing to validate the solution’s correctness and efficiency.
    \end{itemize}
\end{enumerate} \\
\hline
\end{tabular}
\caption{Examples of Applying the Agentic Workflow in Different Scenarios}
\label{tab:examples}
\end{table*}

By integrating these components, the LLM Agentic Workflow not only enhances the learning experience but also equips students with the necessary skills to tackle real-world programming challenges. This approach underscores the transformative potential of LLMs in education, fostering a more interactive, supportive, and effective learning environment.



% llm + langchain
To solve our research problem, we aim to leverage the LLMs with Retrieval-Augmented Generation (RAG) techniques, which is the process of optimizing the output of a large language model, so it references an authoritative knowledge base outside of its training data sources before generating a response. RAG extends the already powerful capabilities of LLMs to specific domains such as course learning materials, instructor's sylabus without the need to retrain the model. It is a cost-effective approach to improving LLM output so it remains relevant, accurate, and useful in various contexts. This approach sheds light on the relationship between the formulation of prompts and the generative AI.

% \begin{figure}[ht]
% \includegraphics[width=8cm]{images/flowchart_model.png}
% \caption{Flowchart illustrating the model design's iterative code generation and evaluation process.}
% \label{fig:flowchart_model}
% \end{figure}

\begin{figure*}[ht]
\centering
\includegraphics[width=16cm]{images/flowchart_model.png}
\caption{Flowchart illustrating conversational sequence of the model design.}
\label{fig:flowchart_model}
\end{figure*}

We present a structured flowchart, as depicted in Figure. \ref{fig:flowchart_model}, depicting the architecture of a conversational agent, leveraging Retriever-Augmented Generation (RAG) to simulate the educational interplay between a student and a Language Learning Model (LLM). The chart delineates roles, interaction phases, and a guiding document framework, ensuring that the chatbot’s responses are not only contextually pertinent but also pedagogically sound.

\subsection{Roles}
\begin{itemize}
    \item \textbf{Student (User)}: They engage with the chatbot by posing programming inquiries.
    \item \textbf{Instructor}: Provides pedagogical directives to the LLM, typically sourced from course-related materials.
\end{itemize}

\subsection{User Interaction Process}
\begin{itemize}
    \item \textbf{Initiation (Question}): The dialogue begins when the student submits a coding query.
    \item \textbf{Sequential Processing (Chain)}: This denotes a series of interactions or processing stages.
    \item LLM Engagement: Here, the RAG model reformulates the query, using dialogue history for an enhanced understanding.
    \item \textbf{Query Refinement (Rephrased Question)}: The LLM offers a polished version of the initial inquiry.
    \item \textbf{Instructional Resources (Relevant Documents}): Course materials curated by the instructor, fetched in response to the refined query.
    \item \textbf{Response Formulation (Answer Rephrased Question Using Documents}): Crafting the reply utilizing the sourced educational content.
    \item \textbf{Final Response (Answer)}: The definitive answer delivered to the student.
    \item \textbf{Dialogue Continuity (Multi-rounds Update)}: Indicates the chatbot’s capability for ongoing interaction, refining responses through successive dialogue turns.
\end{itemize}

\subsection{Document-Guided Framework}
The chatbot adheres to an instructional rubric, fostering constructive educational interactions:
\begin{enumerate}
    \item \textbf{Problem Assessment}: Begins with categorizing the coding dilemma, thereby employing pertinent problem-resolution techniques. Recognizing the essence of the challenge is vital for its decomposition into solvable segments, simplifying intricate issues. This phase also includes forecasting typical obstacles, such as the selection of data structures or the application of algorithms in Python.
    \item \textbf{Pseudo-code Drafting}: Transitions to delineating an abstract representation of the solution. This crucial phase paves the way for the coding journey, emphasizing logic over syntax and promoting a progressive problem-solving mindset.
    \item \textbf{Code Review}: Focuses on critiquing the user’s initial code, examining the logical framework and data structure utilization while ensuring syntactical conformity. It involves delivering pointed advice for refinement, assisting the user in enhancing their coding acumen.
    \item \textbf{Progressive Refinement}: Entails the ongoing evaluation of user code revisions, providing insightful feedback and suggestions for advancements. This reinforces the learning cycle, encouraging the production of high-caliber code.
    \item \textbf{Exercise Conclusion}: Culminates the session by either commending the student’s success or offering further assistance. If needed, a complete, annotated code solution is presented, ensuring an all-encompassing educational experience.
    \item \textbf{Session Recap and Motivation}: Summarizes the pivotal concepts and challenges addressed, offering a succinct retrospective of the learning episode. It concludes with affirmations and motivation for continued engagement with coding exercises.
\end{enumerate}

This delineation underscores a methodical approach to inquiry resolution, wherein the chatbot augments its responses with instructional content and a predefined educational protocol. The RAG structure employs a retrieval methodology to fortify the response generation, integrating knowledge from external documents, yielding responses of higher accuracy and contextual relevance. This framework is conducive to a dialogic engagement, reminiscent of real-world pedagogical interactions, where a student’s coding quandaries are addressed through a systematic, stepwise mentorship.



% Detailed elucidation on prompt configurations and examples is in our Appendix, as referenced in \ref{section:prompt}.




% \begin{table}
% \centering
% \caption{User Prompt for Single-Round Dialog Model}
% \begin{tabular}{|p{1.2cm}|p{2.5cm}|p{3.5cm}|}
% \hline
% \textbf{Model} & \textbf{System Prompt} & \textbf{User Prompt} \\
% \hline
% Model 1 & \multirow{3}{3cm}{\textit{System Prompt} (See Appendix~\ref{section:prompt})} & Coding Question\\
% \cline{1-1}\cline{3-3}
% Model 2 & & Coding Question + Test Cases\\
% \cline{1-1}\cline{3-3}
% Model 3 & & Coding Question + Test Cases + General Guidelines\\
%  \cline{1-1}\cline{3-3}
% Model 4 & & Coding Question + Test Cases + Specific Guidelines\\
% \hline
% \end{tabular}
% \label{tab:single_round_prompt}
% % Directly under the table
% \\\vspace{2mm} % Adjust the space as needed
%  \raggedright
% * Please refer to Section~\ref{subsec:prompt_config} for the meaning of General and Specific Guideline. 
% \end{table}









==> sections/notes.tex <==



==> sections/problem_formulation.tex <==
\section{Problem Statement}
\label{section:problem_statement}
% Our research seeks to address the following challenges in the domain of programming education enhanced by Large Language Models (LLMs):

% % which kind of system we plan to build
% \begin{itemize}
%     \item \textbf{Integration of LLMs in Educational Settings}: Identifying effective strategies for employing LLMs in programming education to leverage their potential for generating high-quality Python code.

%     \item \textbf{Augmented Coding Guidelines}: Developing and integrating enhanced coding guidelines to improve the efficiency, readability, and adherence to Pythonic principles in code generated by LLMs.

%     \item \textbf{Prompt Engineering and Iterative Refinement}: Investigating the impact of prompt engineering on the quality of LLM-generated code through an iterative process of refinement and evaluation.

%     \item \textbf{Academic Contribution and Educator Support}: Contributing to the academic discussion on AI-assisted programming education and offering practical insights for educators on integrating LLMs into computer science curricula effectively.

% \end{itemize}

% These challenges underline the need for a nuanced approach to harnessing LLMs in programming education, aiming to transform the learning experience and prepare students for the dynamic software development industry.


\textcolor{red}{moving this content into the problem formulation, we need to make the introduction being short.  In the discussion, we need to pick up one or more problem(s) to illustrate what we are taking about - the pain points of the students and the teacher.}

% Explain the flowchart of new learning approach using LLMs
We present an in-depth depiction of the adaptable learning process facilitated by LLMs in computer programming education. The objective is to establish a systematic framework for enhancing the learning process of computer programming with a focus on high-quality code development. The methodology is structured to incrementally develop the learner's capability to dissect complex coding problems into smaller, manageable tasks, thereby promoting analytical thinking and problem-solving proficiency. Our system aims to incrementally nurture the learner's ability to evaluate, design, and execute coding solutions that adhere to standards of efficiency, readability, and robustness, ensuring a comprehensive understanding of programming concepts.

\begin{enumerate}
    \item \textbf{Problem Examination}: Begin by identifying the type of coding problem, drawing from the knowledge of different categories. This helps in applying the correct problem-solving strategies, such as selecting suitable algorithms or performing logical analyses. Understanding the problem fully is crucial for breaking it down into manageable components, which can simplify complex issues. Additionally, anticipate potential challenges like choosing the right data structures or implementing algorithms in Python, as these are common hurdles that could impact the solution.

    \item \textbf{Pseudo-code Development}: After grasping the problem's nature, provide a simplified and abstract pseudocode. This step is vital as it lays out a roadmap for the actual coding process, allowing the user to focus on the logic before diving into the syntax. Encourage the user to start writing their code based on this pseudocode, promoting an iterative approach to problem-solving.

    \item \textbf{Code Evaluation}: Evaluate the user's initial code, focusing on the accuracy of its logical structure and the effective use of data structures, while ensuring it adheres to syntactic norms. Offer specific feedback for improvement, guiding the user to refine their code. This iterative process helps in honing their coding skills and aligning their work with best practices.

    \item \textbf{Iterative Improvement}: Continue to assess revised versions of the user’s code, providing constructive feedback and suggestions for enhancement. This step reinforces the learning process and encourages the user to strive for high-quality code, reflecting best practices and logical precision.

    \item \textbf{Concluding the Exercise}: If the user's code meets the expected standards, acknowledge their success and wrap up the session. If the code still needs improvement, ask if they want the complete solution. If they agree, provide a detailed code solution with explanations, facilitating a comprehensive learning experience.

    \item \textbf{Summary and Encouragement}: Summarize the key points and challenges encountered during the session, offering a concise review of the learning journey. Express gratitude and encourage the user to continue exploring and solving coding problems, reinforcing their confidence and interest in programming.
\end{enumerate}

This innovative teaching methodology, employing LLMs as an integral component of the educational toolkit, not only optimizes the learning trajectory for students but also significantly reduces the pedagogic load on instructors, promising an evolution in computer science education.

% highlights
% \subsection{Our Contributions}
In this paper, we present substantial advancements in the domain of AI-facilitated programming education, with a particular emphasis on enhancing Python code generation through the application of Large Language Models (LLMs). Our contributions are multi-faceted and have significant implications for educational technology:
\begin{itemize}
    \item \textbf{Systematic Student Assistance}: We have developed a standardized methodology that employs LLMs to assist students in navigating a variety of programming challenges. This methodology not only aids in understanding complex concepts but also promotes the development of practical coding skills.
    \item \textbf{Authenticity Evaluation Mechanism}: A novel framework has been proposed to assess the authenticity of the solutions provided by users. This framework ensures that the educational process maintains integrity and that students' work is genuinely reflective of their own understanding and abilities.
    \item \textbf{Comprehensive Code Quality Analysis}: We introduce an innovative approach to evaluate the quality of code from multiple perspectives. This includes syntactic correctness, logical accuracy, and adherence to best coding practices, thereby ensuring that students not only write code that works but also adheres to professional standards.
    \item \textbf{LLM-Powered Chatbot for Education}: We have designed and implemented a chatbot powered by LLMs, specifically tailored for educational purposes. This chatbot acts as an interactive tool that facilitates learning through dynamic conversation, real-time feedback, and personalized tutoring, thereby revolutionizing the traditional programming education landscape.
\end{itemize}





==> sections/related_work.tex <==
\section{Related Work}\label{section:related_work}
% need to re-write and update

% llm in education & development
Recent research in the educational sector has prominently featured the application of Large Language Models (LLMs) to enhance learning outcomes, particularly in the programming domain \cite{denny2023computing}. This review synthesizes findings from key studies that illustrate the diverse roles LLMs play in education, from interactive assistance in computer science courses to the evaluation of programming skills. Murr et al.\cite{murr2023testing} focused on the effectiveness of LLMs in generating code, emphasizing the critical role of prompt specificity. Many studies have demonstrated the efficacy of integrating AI code generators in introductory programming courses, as evidenced by research conducted by Finnie et al.\cite{finnie2022robots}, Hellas et al.\cite{hellas2023exploring}, and Kazemitabaar et al.\cite{kazemitabaar2023studying}. In addition, Kiesler and Schiffner\cite{kiesler2023large} assessed the capabilities of ChatGPT-3.5 and GPT-4 in solving introductory Python programming tasks sourced from CodingBat. Pearce et al.\cite{pearce2022pop} explored the application of LLMs in reverse engineering tasks and exhibited promising results. Supporting discussions on LLMs' application in programming education, particularly with development assistant, additional references such as Asare et al.\cite{asare2023github}, Pearce et al.\cite{pearce2022asleep}, Dakhel et al.\cite{dakhel2023github} and Denny et al. \cite{denny2023chat} provide insights into the integration of AI tools within software development environments. These studies collectively underscore the transformative impact of LLMs on programming education, suggesting avenues for future research in optimizing their use for educational enhancement and addressing broader software development challenges \cite{chen2021evaluating}.

% research gap: issue in LLMs generated code
While LLMs were impressively successful in generating code for different purpose in education and production, they stumbled when confronting real-world security and risks concerns.
Bommasani, R., et al. \cite{bommasani2021opportunities} examine the potential and risks associated with LLMs and highlights their content creation capabilities and warns about potential issues like bias, misinformation, and homogenization. Dakhel et al.~\cite{dakhel2023effective} leveraged LLMs for generating unit tests in software development.

% research gap: prompt engineering to address the issue
% \subsection{Comparative Analysis and Experimental Design}
% For the experimental design aspect, seek papers that detail the setup and methodology for evaluating LLMs in code generation tasks, including the use of prompt engineering and tripartite prompting systems. Research leveraging coding problems from platforms like LeetCode can provide benchmarks for comparison.

To overcome the inaccurate response from LLM, a new discipline or guideline called 'Prompt Engineering', which includes specific strategies for maximizing the capability of LLM, applies to us with modification \cite{reynolds2021prompt, liu2023pre}. Reynolds et al. delve into methodologies for leveraging the inherent capabilities of narratives and cultural anchors to intricately encode intentions and strategies, thereby facilitating a structured breakdown of problems into their constituent elements prior to reaching conclusions \cite{reynolds2021prompt}. Expanding upon this notion, Zhou et al. introduce a novel approach termed least-to-most prompting, which systematically deconstructs complex issues into manageable sub-problems, addressing them sequentially to enhance problem-solving efficiency in LLMs \cite{zhou2022least}. Complementing these insights, Wei et al. demonstrate the natural emergence of reasoning capabilities within sizable LLMs through what is known as chain-of-thought prompting. This technique involves the use of select demonstrations that guide the model through a thought process, thereby facilitating the comprehension and solving of tasks \cite{wei2022chain}. In a similar vein, Arora et al. propose an innovative "Ask Me Anything" (AMA) prompting strategy that iteratively employs the LLM itself to reformulate task inputs into a more effective question-and-answer format, thereby significantly augmenting the performance of LLMs \cite{arora2022ask}. Additionally, Ouyang et al. explore the potential of refining language models' task execution and instruction-following capabilities through the integration of human feedback, marking a significant step towards more interactive and adaptive LLMs \cite{ouyang2022training}. The study by White et al.\cite{white2023prompt} on prompt pattern catalog to enhance prompt engineering with ChatGPT provides a comprehensive overview of best practices and patterns in prompt engineering, highlighting its importance in optimizing LLM outputs for specific tasks.

% evaluation of code quality
% Investigate studies that focus on evaluating the quality of code generated by AI, including aspects like readability, efficiency, and adherence to coding standards. Look for papers that apply third-party assessment methods or develop novel frameworks for objectively measuring code quality.
% Explore research on how transfer learning techniques can be applied to LLMs to improve the quality of generated code, especially in comparison to zero-shot learning scenarios. Studies that categorize coding problems by algorithmic efficiency, memory optimization, and accuracy, and that demonstrate fine-tuning LLMs for specific coding challenges, would be particularly relevant.

The code quality generated by LLMs holds paramount importance in applications spanning educational contexts and real-world production environments and many code evaluation studies have been introduced. Hendrycks et al. \cite{hendrycks2021measuring} unveiled APPS, a benchmark specifically designed for code generation tasks. This benchmark assesses the capability of models to interpret arbitrary natural language specifications and produce Python code that meets the specified requirements. Furthermore, Chen et al. \cite{chen2021evaluating} introduced HumanEval, an innovative evaluation set aimed at measuring the functional correctness of programs synthesized from docstrings. Xu et al. \cite{xu2022systematic} conducted a comprehensive assessment of the largest code-generating models available, spanning multiple programming languages. They introduced a novel model, PolyCoder, which demonstrated superior performance in generating C programming code, outperforming its counterparts. Liu et al. \cite{liu2023your} developed EvalPlus, a comprehensive framework for the evaluation of code synthesis. This framework is meticulously designed to benchmark the functional correctness of code generated by LLMs with a high degree of rigor. White et al. \cite{white2023chatgpt} presented a more systematic methodology for the cataloging of software engineering patterns. This study classifies various patterns and delves into numerous prompt strategies that have been employed to enhance code quality and system design. In a comparative study, Murr et al. \cite{murr2023testing} analyzed the efficacy of code produced by different LLMs across 104 customized Python challenges, utilizing widely recognized metrics such as the pass rate for assessment. 


% \subsection{Quantitative Analysis Methods}
% Look for studies employing BERT-based models or other quantitative analysis techniques to evaluate code quality. Research that examines the impact of different prompt configurations on the generated code's quality will be crucial for supporting the paper's findings.

Beyond conventional methodologies, deep learning techniques have increasingly been applied to the evaluation of code. Kanade et al. \cite{kanade2020learning} explored the capabilities of a finely tuned CuBERT model, revealing that it surpasses traditional methods in source code evaluation. This advantage was observed even with limited training and a smaller number of labeled examples. Ciniselli et al. \cite{ciniselli2021empirical} presented an empirical study employing a RoBERTa model to assess its efficiency in code completion tasks from various angles. The findings indicate that BERT-based models are a promising avenue for enhancing code completion capabilities. Wang et al. \cite{wang2023analyzing} proposed an approach for the automatic assessment of code quality using a BERT model that has been meticulously fine-tuned with specific datasets, offering a groundbreaking perspective on the evaluation of code quality.


%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> sections/result_analysis.tex <==
\section{Experiments and Result Analysis}
\label{section:result_analysis}

\subsection{Dataset}
There are many different sources or coding question banks (benchmarks) to test the ability of AI code generation. In our research, we identified LeetCode~\footnote{https://leetcode.com/} as our experiment code question dataset, owing to its comprehensive range of well-defined and real-world-relevant programming problems. The structured nature of these problems facilitates the AI's processing and solution generation, providing a consistent benchmark for performance analysis. Furthermore, LeetCode's educational utility is significant; it offers students a practical application of theoretical concepts, enhancing learning through exposure to diverse problem-solving techniques. The platform's extensive user community contributes to a dynamic feedback loop, enriching both AI development and educational practices. These attributes collectively establish LeetCode as a valuable resource for advancing and assessing both AI code generation capabilities and pedagogical methods in computer science education.

In summary, we chose and collected LeetCode questions 1 - 100 as our prompt questions. The dataset contains both questions and testing cases. The following is an example of the question. 

\noindent\fbox{%
    \parbox{\linewidth}{%
    \textbf{Problem ID (PID): 1} \\
    
    \textbf{Problem Content:} Given an array of integers nums and an integer target, return indices of the two numbers such that they add up to target. You may assume that each input would have exactly one solution, and you may not use the same element twice. You can return the answer in any order. \\
    
    \textbf{Test Input:}
    \begin{align*}
        \texttt{nums        } &= [2,7,11,15], \\
        \texttt{\space \space  target} &= 9
    \end{align*}
    \textbf{Test Output:} [0,1]
}%
}


\subsection{LLM Models}
This study conducts a comparative analysis of three eminent LLMs: ChatGPT 3.5\footnote{https://help.openai.com/en/articles/6783457-what-is-chatgpt}, ChatGPT 4\footnote{https://openai.com/research/gpt-4}, and Gemini Pro\footnote{https://blog.google/technology/ai/google-gemini-ai/}. Detailed configurations of these models are delineated in the Appendix under the "Hyper-parameter Details." Initially, the investigation evaluates the proficiency of ChatGPT 4 in processing singular interaction prompts. Subsequently, it extends to assess and juxtapose the efficacy of all three models in managing multi-turn user interactions.

Within the domain of LLMs, such as the entity engaged in the current interaction, the terminologies "system prompts" and "user prompts" delineate distinct categories of input stimuli instrumental in directing the model's output generation.

\begin{itemize}
    \item \textbf{System prompt}: is predefined inputs or instructions that are part of the model's design, which help guide the model in generating responses or performing tasks. These elements serve to orient the model towards generating responses or executing tasks with enhanced precision. Such prompts are not introduced by the model's users but are embedded within the system's infrastructure to augment functionality or elevate performance across designated tasks.
    \item \textbf{User prompts}: are the questions, commands, or statements that users input into the system to initiate a response from the LLM. In essence, this encompasses the textual or verbal input furnished by the user to the model.
\end{itemize}

\subsection{LLM Chains}

\subsection{ChatBot Demo}





==> sections_cyber/curriculum_old.tex <==
\section{Challenges and Opportunities for Cybersecurity Education in Non-Traditional Universities}
\section{Challenges for Cybersecurity Education with Diverse Student
Body}


In this section, we delve into the specific challenges and opportunities associated with implementing a cybersecurity education program at a university with a diverse of student body, using Mercy University as a representative case study. Our exploration is structured into three detailed subsections. The first subsection will provide an overview of the student demographic at Mercy University. An overview of their cybersecurity program, and a comprehensive examination of the curriculum, career paths, and skills developed. Additionally, we will highlight the university's industry connections and networking opportunities that align with market needs and career goals. The second subsection will address the diverse skill requirements necessary to meet varying market demands, the sources of cybersecurity knowledge, and the specific math and programming skills essential for effective cybersecurity education, with a focus on algorithm development for cyber-attack detection. The third subsection will summarize the primary pain points encountered in cybersecurity education, drawing from the insights gathered throughout the case study. 


\begin{figure*}[ht]
\centering
\includegraphics[width=14cm]{images/ProgramMap.png}
\caption{Cybersecurity Degree Program Map (\#: Pain Points from Fig. \ref{fig:PainPoint})}
\label{fig:ProgramMap}
\end{figure*}


\begin{comment}



\subsection{Diverse Student Body - Demographics and Challenges}
Mercy University, previously known as Mercy College, has a mission to transform lives through higher education by providing liberal arts and professional programs in personalized and high-quality learning environments. The university aims to prepare students for rewarding careers, lifelong learning, and ethical and responsible actions in a changing world. 


{\color{red} 
Let us move the explain of traditional and non-traditional outside of the figure, and enlarge the figure as big as possible. (say the value can be part of the out circle.}

% roadmap of program -> facing difficulty -> painpoints

\subsubsection{Demographic Analysis}

\begin{figure}[ht]
\centering
\includegraphics[width=8.5cm]{images/DemographicDistribution.png}
\caption[Caption for LOF]{Student Demographic Distribution (Ethnic \& Age Groups)~\protect\footnotemark}
\label{fig:DemographicDistribution}
\end{figure}

\footnotetext{https://www.collegefactual.com/colleges/mercy-college/student-life/diversity}


This section presents a demographic analysis of the student population at Mercy University, with a particular focus on non-traditional students. For this analysis, non-traditional students are defined from two perspectives: (1) racial or ethnic group, and (2) age group.

In contrast to the broader U.S. demographic, where the White non-Hispanic population constitutes 57.8\% \cite{ethnicitypopulation21}, at Mercy University, this group represents only 23.5\% of the student body. The demographic breakdown at Mercy University highlights a richly diverse student population, as illustrated in Figure~\ref{fig:DemographicDistribution}. The data reveals that the largest segment of students identifies as Hispanic or Latino, accounting for 43.1\% of the total enrollment. This is followed by Black or African American students, who comprise 24.6\%, and White students at 23.5\%. Asian students make up 5.8\% of the population, while other ethnic groups, including those identifying as Two or More Races and Native Hawaiian or Other Pacific Islanders, represent 3\%. This demographic distribution underscores the university’s role as an educational institution that caters to a broad spectrum of society, reflecting the defining characteristics of non-traditional universities. Such institutions typically attract students from diverse backgrounds, providing educational opportunities to those who might not follow conventional pathways to higher education. The diversity within the student body presents both challenges and opportunities: educational programs must be tailored to address the varied cultural, socio-economic, and educational needs of these groups, while also leveraging their diverse perspectives to enhance the learning experience.

Similarly, non-traditional students can also be identified by age, with traditional students typically aged 18-24 and non-traditional students defined as those aged 25 and over \cite{traditionstudent24}. The age distribution at Mercy University further highlights its non-traditional nature, with 47.9\% of students falling into the non-traditional age category. The student population is distributed across various age groups, with the largest cohorts being those aged 25-29, comprising 19.8\% of the student body, and those aged 35 and over, representing 18.0\%. This age diversity is indicative of the flexible learning paths that non-traditional universities offer. Many students at Mercy University likely balance their studies with work, family responsibilities, or other personal commitments. This demographic is typical of adult learners who return to education later in life or those who seek to balance education with other life obligations. Such students may have limited time to dedicate to their studies due to external constraints, making the adoption of scalable and personalized learning tools, such as LLMs, particularly beneficial.

\subsubsection{Cybersecurity Program at Mercy University}


Mercy University's cybersecurity program offers a comprehensive blend of theoretical and practical courses designed to equip students with the necessary skills for the field. The curriculum includes foundational courses in computer science, mathematics, and specialized cybersecurity topics. These courses are complemented by hands-on labs, capstone projects, and internships that provide real-world experience.

% Mercy University offers comprehensive programs in cybersecurity that prepare students for various career paths in the field. These programs are designed to provide both theoretical knowledge and practical skills needed to excel in cybersecurity roles. Graduates from these programs are well-prepared for various roles such as information security analyst, IT auditor, and network security administrator. The program boasts a high job growth rate of 32\% by 2028, with an average salary of \$122,000 for information security analysts in New York.

% Mercy University is designated as a National Center of Academic Excellence in Information Assurance Education by the NSA and DHS, which underscores the quality and relevance of its cybersecurity programs



\subsubsection{Programs and Curriculum}
Here's how the cybersecurity education at Mercy University aligns with industry requirements and career paths:

\begin{itemize}
    \item \textbf{Degree Programs}: Mercy University offers bachelor's and master's degrees in cybersecurity, covering topics such as network security, ethical hacking, incident response, and cybersecurity governance.
    \item \textbf{Certifications}: The curriculum includes preparation for industry-recognized certifications like CompTIA Security+, Certified Information Systems Security Professional (CISSP), and Certified Ethical Hacker (CEH). These certifications are crucial for validating skills and enhancing employability in the cybersecurity field \cite{coursera2024} \cite{eccu2024}.
    \item \textbf{Practical Experience}: Emphasis is placed on hands-on learning through labs, simulations, and real-world projects. Practical experience is essential for understanding the complexities of cybersecurity threats and responses \cite{coursera2024} \cite{caltech2024}.
\end{itemize}

\end{comment}


\subsection{Career Paths Supported by Mercy University's Cybersecurity Programs}

\begin{itemize}
    \item \textbf{Cybersecurity Analyst}: Training includes monitoring and analyzing security threats, identifying vulnerabilities, and responding to incidents. The curriculum covers network security, threat intelligence, and incident management.
    \item \textbf{Ethical Hacker/Penetration Tester}: Students are trained in ethical hacking tools and techniques, preparing them to simulate cyber attacks and identify security weaknesses.
    \item \textbf{Security Consultant}: Coursework in risk assessment, compliance, and strategic planning equips students to provide expert cybersecurity advice to organizations.
    \item \textbf{Incident Responder}: Focus on incident response and forensic analysis prepares students to handle security breaches effectively and implement preventive measures \cite{isc22024} \cite{eccu2024}.
    \item \textbf{Security Architect}: Courses on security frameworks, system design, and risk management help students design and implement secure systems and infrastructures.
\end{itemize}

\subsection{Skills Developed}

\begin{itemize}
    \item \textbf{Technical Skills}: Students gain proficiency in coding (Python, Java, SQL), cloud security platforms (AWS, Azure, Google Cloud), and network security tools. These skills are fundamental for various cybersecurity roles \cite{coursera2024} \cite{cyberseek2024}.
    \item \textbf{Soft Skills}: Emphasis on communication, critical thinking, and teamwork, as these are vital for collaborating with different teams and stakeholders in cybersecurity roles.
    \item \textbf{Continuous Learning}: The dynamic nature of cybersecurity necessitates ongoing education. Mercy University encourages students to stay updated with the latest industry trends, emerging threats, and new technologies through continuous learning opportunities and advanced coursework \cite{coursera2024} \cite{isc22024}.
\end{itemize}

\subsection{Industry Connections and Networking}

Mercy University facilitates connections with industry professionals through internships, career fairs, and networking events. These opportunities allow students to gain real-world experience and build professional relationships that are crucial for career advancement in cybersecurity \cite{eccu2024} \cite{cyberseek2024}.

\subsection{Market Needs and Career Goals}
The demand for cybersecurity professionals continues to grow as cyber threats become more sophisticated and pervasive. Industries such as finance, healthcare, government, and technology are increasingly seeking skilled cybersecurity experts to protect sensitive information and infrastructure. According to labor market projections, the cybersecurity job market is expected to grow significantly in the coming years, with roles such as security analysts, ethical hackers, digital forensics experts, and cybersecurity consultants being in high demand.

Students entering the cybersecurity field often have diverse career goals, ranging from technical positions such as penetration testers and security engineers to strategic roles like security managers and consultants. Personalized education is crucial to cater to these varying career aspirations. By tailoring the curriculum to individual needs, educators can help students acquire the specific skills required for their desired career paths, thereby enhancing their employability and career satisfaction.




% Students Challenges (Pain Points)
\begin{figure*}[ht]
\centering
\includegraphics[width=16cm]{images/PainPoint.png}
\caption{Pain Points (\#1-\#6) in Cybersecurity Education with Diverse Student Body}
\label{fig:PainPoint}
\end{figure*}


\subsection{Skill Requirements and Educational Strategies}

\subsubsection{Diversity of Skills Requirement for Different Market Needs}
Cybersecurity is a multidisciplinary field that requires a diverse set of skills. Technical skills such as network security, cryptography, and secure coding are fundamental for most cybersecurity roles. However, soft skills like critical thinking, problem-solving, communication, and teamwork are equally important, especially for roles that involve collaboration and strategic decision-making.

Different industries also have unique cybersecurity needs. For instance, the healthcare sector prioritizes data privacy and compliance with regulations like HIPAA, while the financial sector focuses on fraud prevention and secure transaction processing. Personalized education allows students to develop industry-specific knowledge and skills, making them more adaptable and valuable in the job market.

\subsubsection{Sources of Cybersecurity Knowledge}
We address the sources of cybersecurity knowledge, categorizing them into academic resources, industry publications, online courses, and practical experiences. This categorization helps in structuring the curriculum to ensure a well-rounded education that covers both theoretical knowledge and practical skills. By leveraging LLMs and RAG, educators can provide students with access to the most current and relevant information, fostering a deeper and more comprehensive understanding of cybersecurity concepts.

\subsubsection{Math Requirements for Cybersecurity}
A solid understanding of basic math is essential for students pursuing a major in cybersecurity. Math skills underpin many aspects of cybersecurity, from cryptography to data analysis. We demonstrate how the agentic workflow can provide personalized support to help students develop these foundational skills. By offering personalized tutoring, generating practice problems, and providing step-by-step solutions, LLMs can help students build a strong mathematical foundation, which is critical for their success in more advanced cybersecurity topics.

\subsubsection{Programming Skills and Algorithm Development for Cyber-Attack Detection}
This section focuses on the importance of basic programming skills and algorithm development in the context of cybersecurity. Students learn to develop algorithms for detecting and mitigating cyber-attacks, understanding the principles behind various security measures. We discuss common pain points in learning programming and strategies to overcome these challenges, emphasizing the iterative problem-solving approach facilitated by LLMs.

%\subsection{Summary of Pain Points in Cybersecurity Education}

In this section, we address two primary challenges faced by cybersecurity students at non-traditional universities: mentorship and accessibility challenges, and career support and certification gaps. These challenges significantly impact the quality of education and the preparedness of students for the cybersecurity workforce. Figure \ref{fig:PainPoint} illustrates the intricate connections between these challenges, emphasizing the critical need for comprehensive solutions to enhance the educational experience and career readiness of students.

\begin{enumerate}
    \item \textbf{Mentorship and Accessibility Challenges}: This category groups issues related to the availability and quality of mentorship, as well as the flexibility of educational resources. These factors are crucial in shaping a student's academic experience and access to knowledge.
    \item \textbf{Career Support and Certification Gaps}: These pain points specifically address the challenges students face in preparing for their professional careers, including the need for proper guidance and relevant certifications.
    \item \textbf{Lack of Cutting-edge Knowledge}: This category highlights the time constraints on both students and educators to master cutting-edge knowledge for both academic and professional demands.
\end{enumerate}

% introduce why we introduce our model
Therefore, the importance of our research lies in its focus on non-traditional universities like Mercy University, which represent a significant portion of higher education institutions in the United States. Unlike well-funded research institutions, these universities often operate with limited resources, yet serve a substantial student population. Addressing the unique challenges faced by these institutions is crucial for enhancing the quality of cybersecurity education and ensuring students are well-prepared for the workforce. Our research emphasizes the critical need for innovative solutions to overcome mentorship, accessibility, career support, and certification gaps. One such solution is the introduction of a 24/7 mentoring system. This system can provide continuous support and personalized guidance, alleviating the strain on limited human resources and ensuring that students have access to the necessary tools and information at any time.

==> sections_cyber/discussion.tex <==
\section{Discussion}
\label{section:discussion}

% merged into conclusion to reduce page limit

==> sections_cyber/literacture_review.tex <==
\section{Literature Review}

% to-do, place-holder
This section provides a comprehensive literature review of cybersecurity education and the use of Large Language Models (LLMs) in higher education. We examine existing research on effective teaching methods in cybersecurity, the integration of practical skills in academic programs, and the challenges faced by educators and students. The review also covers studies on the application of LLMs in education, highlighting their potential to enhance learning experiences, provide personalized support, and improve educational outcomes.

\subsection{Evaluating the Effectiveness of LLMs in Introductory Computer Science Education: A Semester-Long Field Study}
This study investigates the impact of LLMs on students' performance and engagement in an introductory computer science course over a semester. The research found that students who used LLMs as part of their learning process showed significant improvements in understanding complex programming concepts and problem-solving skills. The study highlights the advantages of using LLMs for providing instant feedback, personalized tutoring, and practical coding assistance, which collectively enhance the learning experience and help students overcome common hurdles in computer science education \cite{fieldstudy2023}.

\subsection{AI-Assisted Learning with ChatGPT and Large Language Models: Implications for Higher Education}
This paper explores the broader implications of integrating AI-assisted learning tools, specifically ChatGPT and other LLMs, into higher education. The authors discuss the potential benefits of these technologies, such as personalized learning, increased accessibility to educational resources, and the ability to tailor educational content to individual student needs. They also address potential challenges, including ethical considerations, the need for faculty training, and the importance of maintaining academic integrity. The paper provides a comprehensive overview of how LLMs can be effectively used to enhance educational outcomes and suggests best practices for their implementation \cite{chatgpt2024}.

\subsection{Effective Teaching Methods in Cybersecurity Education}
Cybersecurity education poses unique challenges due to the rapidly evolving nature of cyber threats and the need for both theoretical knowledge and practical skills. Effective teaching methods identified in the literature include hands-on labs, simulation exercises, and real-world problem-solving scenarios. These methods help bridge the gap between theoretical concepts and practical application, preparing students for the complexities of cybersecurity work. Additionally, interdisciplinary approaches that integrate knowledge from fields such as computer science, law, and psychology are emphasized as essential for a well-rounded cybersecurity education \cite{cyberteachingmethods2021}.

\subsection{Integration of Practical Skills in Academic Programs}
Several studies emphasize the importance of integrating practical skills into cybersecurity academic programs. Practical skills development can be achieved through internships, capstone projects, and collaboration with industry partners. These opportunities provide students with real-world experience and enhance their employability. The literature suggests that programs that effectively blend theoretical instruction with practical application produce graduates who are better equipped to handle the demands of the cybersecurity industry \cite{practicalskills2019}.

\subsection{Challenges Faced by Educators and Students in Cybersecurity Education}
Educators in cybersecurity face numerous challenges, including keeping curriculum content current with the latest threats and technologies, providing adequate hands-on experiences, and addressing the diverse backgrounds and skill levels of students. Students, on the other hand, often struggle with the complexity of cybersecurity concepts and the need for continuous learning to stay updated with the field's rapid advancements. The literature highlights the need for adaptive teaching methods and resources that can cater to individual learning paces and preferences \cite{cyberchallenges2020}.

\subsection{Application of LLMs in Education}
The application of LLMs in education is a growing area of interest, with studies showing promising results in various contexts. LLMs can provide personalized learning experiences by adapting content to the individual needs of students, offering real-time assistance, and generating customized practice problems and explanations. These capabilities make LLMs valuable tools for enhancing student engagement and understanding, particularly in challenging subjects like cybersecurity. Additionally, LLMs can support educators by automating administrative tasks, such as grading and providing feedback, allowing them to focus more on teaching and student interaction \cite{llmeducation2023}.

\subsection{Implications and Best Practices for Implementing LLMs in Education}
While the potential benefits of LLMs in education are significant, their implementation must be carefully managed to address potential challenges. Ethical considerations, such as ensuring data privacy and preventing academic misconduct, are critical. Training for educators on how to effectively integrate LLMs into their teaching practices is also essential. The literature suggests that a blended approach, combining traditional teaching methods with AI-assisted tools, may offer the best results. Continuous evaluation and adaptation of these tools are necessary to ensure they meet the evolving needs of students and educators \cite{bestpractices2022}.



==> sections_cyber/try.tex <==
\subsection{Cybersecurity at Mercy University}

Mercy University offers comprehensive programs in cybersecurity that prepare students for various career paths in the field. These programs are designed to provide both theoretical knowledge and practical skills needed to excel in cybersecurity roles. Here's how the cybersecurity education at Mercy University aligns with industry requirements and career paths:

\subsection{Programs and Curriculum}

\begin{itemize}
    \item \textbf{Degree Programs}: Mercy University offers bachelor's and master's degrees in cybersecurity, covering topics such as network security, ethical hacking, incident response, and cybersecurity governance.
    \item \textbf{Certifications}: The curriculum includes preparation for industry-recognized certifications like CompTIA Security+, Certified Information Systems Security Professional (CISSP), and Certified Ethical Hacker (CEH). These certifications are crucial for validating skills and enhancing employability in the cybersecurity field \cite{coursera2024} \cite{eccu2024}.
    \item \textbf{Practical Experience}: Emphasis is placed on hands-on learning through labs, simulations, and real-world projects. Practical experience is essential for understanding the complexities of cybersecurity threats and responses \cite{coursera2024} \cite{caltech2024}.
\end{itemize}

\subsection{Career Paths Supported by Mercy University's Cybersecurity Programs}

\begin{itemize}
    \item \textbf{Cybersecurity Analyst}: Training includes monitoring and analyzing security threats, identifying vulnerabilities, and responding to incidents. The curriculum covers network security, threat intelligence, and incident management.
    \item \textbf{Ethical Hacker/Penetration Tester}: Students are trained in ethical hacking tools and techniques, preparing them to simulate cyberattacks and identify security weaknesses.
    \item \textbf{Security Consultant}: Coursework in risk assessment, compliance, and strategic planning equips students to provide expert cybersecurity advice to organizations.
    \item \textbf{Incident Responder}: Focus on incident response and forensic analysis prepares students to handle security breaches effectively and implement preventive measures \cite{isc22024} \cite{eccu2024}.
    \item \textbf{Security Architect}: Courses on security frameworks, system design, and risk management help students design and implement secure systems and infrastructures.
\end{itemize}

\subsection{Skills Developed}

\begin{itemize}
    \item \textbf{Technical Skills}: Students gain proficiency in coding (Python, C++, SQL), cloud security platforms (AWS, Azure, Google Cloud), and network security tools. These skills are fundamental for various cybersecurity roles \cite{coursera2024} \cite{cyberseek2024}.
    \item \textbf{Soft Skills}: Emphasis on communication, critical thinking, and teamwork, as these are vital for collaborating with different teams and stakeholders in cybersecurity roles.
    \item \textbf{Continuous Learning}: The dynamic nature of cybersecurity necessitates ongoing education. Mercy University encourages students to stay updated with the latest industry trends, emerging threats, and new technologies through continuous learning opportunities and advanced coursework \cite{coursera2024} \cite{isc22024}.
\end{itemize}

\subsection{Industry Connections and Networking}

Mercy University facilitates connections with industry professionals through internships, career fairs, and networking events. These opportunities allow students to gain real-world experience and build professional relationships that are crucial for career advancement in cybersecurity \cite{eccu2024} \cite{cyberseek2024}.

\subsection{Conclusion}

Mercy University's cybersecurity programs are designed to equip students with the knowledge, skills, and practical experience required to succeed in various cybersecurity careers. The university's focus on industry-relevant certifications, hands-on learning, and continuous professional development ensures that graduates are well-prepared to meet the demands of the cybersecurity field. For more details on the programs and career support, you can visit Mercy University's \href{https://www.mercy.edu/academics/programs/cybersecurity}{cybersecurity program page}.

